Distance Dependent Chinese Restaurant Processes

We develop the distance dependent Chinese restaurant process (CRP), a flexible class of distributions over partitions that allows for non-exchangeability. This class can be used to model many kinds of dependencies between data in infinite clustering models, including dependencies across time or space. We examine the properties of the distance dependent CRP, discuss its connections to Bayesian nonparametric mixture models, and derive a Gibbs sampler for both observed and mixture settings. We study its performance with three text corpora. We show that relaxing the assumption of exchangeability with distance dependent CRPs can provide a better fit to sequential data. We also show its alternative formulation of the traditional CRP leads to a faster-mixing Gibbs sampling algorithm than the one based on the original formulation.

==> arxiv-preamble.tex <==
% references

\newcommand{\mysec}[1]{Section~\ref{sec:#1}}
\newcommand{\myapp}[1]{Appendix~\ref{app:#1}}
\newcommand{\myeq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\myeqp}[1]{Eq.~\ref{eq:#1}}
\newcommand{\mychap}[1]{Chapter~\ref{chap:#1}}

% math conveniences

\newcommand{\g}{\,\vert\,}
\newcommand{\E}{\textrm{E}}
\newcommand{\vct}[1]{\textbf{#1}}
\newcommand{\realline}{\mathbb{R}}
\newcommand{\indpt}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\h}[1]{\textrm{H}\left( #1 \right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\R}{\mathbb{R}}

% packages

\usepackage{times} % alt: cmbright
\usepackage{amsmath}
%\usepackage[varg]{txfonts}
\usepackage[top=2.5cm, bottom=2.5cm, left=2.5cm, right=2.5cm]{geometry}
\usepackage{natbib}

\usepackage{amssymb}
% \usepackage{latexsym}
% \usepackage{sectsty}
\usepackage{amsfonts}
\usepackage{epsfig}
\usepackage{url}
\usepackage{rotating}

% paragraph spacing

\setlength{\parindent}{0pt}
\setlength{\parskip}{1ex plus 0.5ex minus 0.2ex}

\usepackage{microtype}

\usepackage{graphicx}

\newcommand{\yrcite}[1]{\citep{#1}}
\newcommand{\myfig}[1]{Figure~\ref{fig:#1}}
\newcommand{\ind}[1]{1[#1]}
\newcommand{\rmnew}{\textrm{new}}
\newcommand{\vw}{\vec{w}}
\newcommand{\Prob}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Pmeasure}{\mathbb{P}}
\newcommand{\DP}{\mathrm{DP}}
\newcommand{\mypar}[1]{\paragraph{#1}}
\usepackage[compact]{titlesec}

\newenvironment{packed_enumerate}{
  \begin{enumerate}
    \setlength{\topsep}{0pt}
    \setlength{\itemsep}{6pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
}{\end{enumerate}}

% this is ued in arxiv-preamble
\usepackage{amsthm}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}


==> diff.tex <==
\section{Distance dependent CRPs}
\label{sec:model}

\begin{figure}[t]
  \begin{center}
    \includegraphics[width=\textwidth]{figs/ddcrp-intuition.pdf}
  \end{center}
  \caption{An illustration of the distance dependent CRP.  The process
    operates at the level of customer assignments, where each customer
    chooses either another customer or no customer according to
    \myeq{dec-crp-prior}.  Customers that chose not to connect to
    another are indicated with a self link The table assignments, a
    representation of the partition that is familiar to the CRP, are
    derived from the customer assignments.\label{fig:tables}}
\end{figure}

\begin{figure*}[htp]
  \begin{center}
  \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{figs/identity.pdf} &
    \includegraphics[width=0.5\textwidth]{figs/window.pdf} \\
    \includegraphics[width=0.5\textwidth]{figs/exponential.pdf} &
    \includegraphics[width=0.5\textwidth]{figs/logistic.pdf}
  \end{tabular}
\end{center}
\caption{Draws from sequential CRPs.  Illustrated are draws for
  different decay functions, which are inset: (1) The traditional CRP;
  (2) The window decay function; (3) The exponential decay function;
  (4) The logistic decay function.  The table assignments
  are illustrated, which are derived from the customer assignments drawn from
  the distance dependent CRP.  The decay functions (inset) are
  functions of the distance between the current customer and each
  previous customer. \label{fig:priors}}
\end{figure*}

The Chinese restaurant process (CRP) is a probability distribution over
partitions~\citep{Pitman:2002}.  It is described by considering a
Chinese restaurant with an infinite number of tables and a sequential
process by which customers enter the restaurant and each sit down at a
randomly chosen table.  After $N$ customers have sat down, their
configuration at the tables represents a random partition.  Customers
sitting at the same table are in the same cycle.

In the traditional CRP, the probability of a customer sitting at a
table is computed from the number of other customers already sitting
at that table.  Let $z_i$ denote the table assignment of the $i$th
customer, assume that the customers $z_{1:(i-1)}$ occupy $K$ tables,
and let $n_k$ denote the number of customers sitting at table $k$.
The traditional CRP draws each $z_i$ sequentially,
\begin{equation}
  p(z_i = k \g z_{1:(i-1)}, \alpha) \propto
  \left\{
    \begin{array}{ll}
      n_k & \textrm{for} \quad k \leq K\\
      \alpha & \textrm{for} \quad k=K+1,
    \end{array}
  \right.
  \label{eq:crp-prior}
\end{equation}
where $\alpha$ is a given scaling parameter.
When all $N$ customers have been seated, their table assignments
provide a random partition.  Though the process is described
sequentially, the CRP is exchangeable.  The probability of a
particular partition of $N$ customers is invariant to the order in
which they sat down.

We now introduce the \textit{distance dependent CRP}.  In this
distribution, the seating plan probability is described in terms of
the probability of a customer sitting with each of the other
\textit{customers}.  The allocation of customers to tables is a
by-product of this representation.  If two customers are reachable by
a sequence of interim customer assignments, then they at the same
table.  This is illustrated in \myfig{tables}.

Let $c_i$ denote the $i$th customer assignment, the index of the
customer with whom the $i$th customer is sitting.  Let $d_{ij}$ denote
the distance measurement between customers $i$ and $j$, let $D$ denote
the set of all distance measurements between customers, and let $f$ be
a decay function (described in more detail below).  The distance
dependent CRP independently draws the customer assignments conditioned
on the distance measurements,
\begin{equation}
  p(c_i = j \g D, \alpha) \propto
  \left\{
    \begin{array}{ll}
      f(d_{ij}) & \textrm{if} \quad j \neq i \\
      \alpha & \textrm{if} \quad i = j.
    \end{array}
  \right.
  \label{eq:dec-crp-prior}
\end{equation}
Notice the customer assignments do not depend on other customer
assignments, only the distances between customers.  Also notice that
$j$ ranges over the entire set of customers, and so any customer may
sit with any other.  (If desirable, restrictions are possible through
the distances $d_{ij}$. See the discussion below of sequential CRPs.)

Each customer's choice of with whom to sit is decoupled from where the
others are sitting.  Customers are still assigned to tables; however,
the table assignments are indirectly determined by the way in which
customers are assigned to each other (again, see \myfig{tables}).
Finally, note that the customer assignments can produce a cycle (e.g.,
customer 1 sits with 2 and customer 2 sits with 1).  This still
determines a valid seating assignment: All customers sitting in a
cycle are assigned to the same table.

By being defined over customer assignments, the distance dependent CRP
provides a more expressive distribution over partitions than models
based on table assignments.  This distribution is determined by the
nature of the distance measurements and the decay function.  For
example, if each customer is time-stamped, then $d_{ij}$ might be the
time difference between customers $i$ and $j$; the decay function can
encourage customers to sit with those that are contemporaneous.  If
each customer is associated with a location in space, then $d_{ij}$
might be the Euclidean distance between them; the decay function can
encourage customers to sit with those that are in
proximity.\footnote{The probability distribution over
  partitions defined by \myeq{dec-crp-prior} is similar to the
  distribution over partitions presented in \cite{Dahl:2008}.  That
  probability distribution may be specified by \myeq{dec-crp-prior} if
  $f(d_{ij})$ is replaced by a \DIFaddbegin \DIFadd{non-negative }\DIFaddend value $h_{ij}$ that satisfies
  a normalization requirement $\sum_{i\ne j} h_{ij} = N-1$ for each $j$.  
  Thus, the model presented in \cite{Dahl:2008} may be understood as a
  normalized version of the distance dependent CRP.  To write this model as
  a distance dependent CRP, take $d_{ij} = 1/h_{ij}$ and $f(d) = 1/d$ (with
  $1/0=\infty$ and $1/\infty=0$), so that $f(d_{ij})=h_{ij}$.}  
For many sets of
distance measurements, the resulting distribution over partitions is
no longer exchangeable; this is an appropriate distribution to use
when exchangeability is not a reasonable assumption.

% Notational differences: in Dahl, $c_i$ is the {\it cluster} to which
% customer $i$ belongs, rather than the {\it customer} to which
% $c_i$ links.

% dmb: !!! (below) where are these assumptions important?  do we need
% to discuss them here?

\paragraph{Decay functions.}  In general, the decay function
mediates how distances between customers affect the resulting
distribution over partitions.  We assume that the decay function $f$ is
non-increasing, takes non-negative finite values, and satisfies
$f(\infty)=0$.  We consider several types of decay as examples, all of which
satisfy these nonrestrictive assumptions.

The \textit{window decay} $f(d) = 1[d<a]$ only considers
customers that are at most distance $a$ from the current customer. The
\textit{exponential decay} $f(d) = e^{-d/a}$ decays the probability of
linking to
an earlier customer exponentially with the distance to the current
customer. The \textit{logistic decay} $f(d) = \exp{(-d + a)} / (1 +
\exp{(-d + a)})$ is a smooth version of the window decay.  Each of these
affects the distribution over partitions in a different way.

\paragraph{Sequential CRPs and the traditional CRP.}  With certain
types of distance measurements and decay functions, we obtain the
special case of \textit{sequential CRPs}.\footnote{Even though the
  traditional CRP is described as a sequential process, it gives an
  exchangeable distribution.  Thus, sequential CRPs, which include
  both the traditional CRP as well as non-exchangeable distributions,
  are more expressive than the traditional CRP.}  A sequential CRP is
constructed by assuming that $d_{ij} = \infty$ for those $j>i$.  With
our previous requirement that $f(\infty) = 0$, this guarantees that no
customer can be assigned to a later customer, i.e., $p(c_i \leq i \g
D) = 1$.  The sequential CRP lets us define alternative formulations
of some previous time-series models.  For example, with a window decay
function and $a=1$, we recover the model studied in~\cite{Ahmed:2008}.  
With a logistic decay function, we recover
the model studied in~\cite{Zhu:2005}.  In our empirical study we will
examine sequential models in detail.

The sequential CRP can re-express the traditional CRP.  Specifically,
the traditional CRP is recovered when $f(d) = 1$ for $d \neq \infty$
and $d_{ij}<\infty$ for $j < i$. To see this, consider the marginal
distribution of a customer sitting at a particular table, given the
previous customers' assignments.  The probability of being assigned to
each of the other customers at that table is proportional to one.
Thus, the probability of sitting at that table is proportional to the
number of customers already sitting there.  Moreover, the probability
of not being assigned to a previous customer is proportional to the
scaling parameter $\alpha$.  This is precisely the traditional CRP
distribution of \myeq{crp-prior}.  Although these models are
the same, the corresponding Gibbs samplers are different (see
\mysec{crp-comparison}).

\myfig{priors} illustrates seating assignments (at the \textit{table}
level) derived from draws from sequential CRPs with each of the decay
functions described above, including the original CRP.  (To adapt
these settings to the sequential case, the distances are $d_{ij} =
i - j$ for $j < i$ and $d_{ij}=\infty$ for $j > i$.)
Compared to the traditional CRP, customers tend to sit at the same
table with other nearby customers.  We emphasize that sequential CRPs
are only one type of distance dependent CRP.  Other distances,
combined with the formulation of \myeq{dec-crp-prior}, lead to a
variety of other non-exchangeable distributions over partitions.

\paragraph{Marginal invariance.}  The traditional CRP is
\textit{marginally invariant}: Marginalizing over a particular
customer gives the same probability distribution as if that customer
were not included in the model at all.  The distance dependent CRP
does not generally have this property, allowing it to capture the way
in which influence might be transmitted from one point to another.
See \mysec{marg} for a precise characterization of the class of
distance dependent CRPs that are marginally invariant.

% Another independent version of this paragraph: Some probabilistic
% models for pairings of covariates with data have the property that
% marginalizing over all the possible observation values for a
% particular covariate gives the same probability distribution over
% the remaining observations as the model with that covariate removed
% entirely.  Many of previous approaches for inducing have this
% property, including the distance dependent Dirichlet process (DDP)
% of [citation], the ordered DP of [citation], [what else].

% Thus, one guide for whether the distance dependent CRP might be a
% useful model in a particular situation is whether or not marginal
% invariance is a reasonable assumption.

To see when this might be a relevant property, consider the goal of
modeling preferences of people within a social network.  The model
used should reflect the fact that persons A and B are more likely to
share preferences if they also share a common friend C.  Any
marginally invariant model, however, would insist that the
distribution of the preferences of A and B is the same whether (1)
they have no such common friend C, or (2) they do but his preferences
are unobserved and hence marginalized out.  In this setting, we might
prefer a model that is not marginally invariant.  Knowing that they
have a common friend affects the probability that A and B share
preferences, regardless of whether the friend's preferences are
observed.  A similar example is 
modeling the spread of disease.  Suddenly discovering a city between
two others--even if the status of that city is unobserved--should
change our assessment of the probability that the disease travels
between them.

We note, however, that if observations are missing then models that
are not marginally invariant require that relevant conditional
distributions be computed as ratios of normalizing constants.  In
contrast, marginally invariant models afford a more convenient
factorization, and so allow easier computation.  Even when faced with
data that clearly deviates from marginal invariance, the modeler may
be tempted to use a marginally invariant model, choosing computational
convenience over fidelity to the data.
% But recall the Emerson quote, ``A foolish consistency is the hobgoblin of little minds.''

\paragraph{} We have described a general formulation of the distance
dependent CRP.  We now describe two applications to Bayesian modeling
of discrete data, one in a fully observed model and the other in a
mixture model.  These examples illustrate how one might use the
posterior distribution of the partitions, given data and an assumed
generating process based on the distance dependent CRP.  We will focus
on models of discrete data and we will use the terminology of document
collections to describe these models.\footnote{While we focus on text,
  these models apply to any discrete data, such as genetic data, and,
  with modification, to non-discrete data as well.  That said,
  CRP-based methods have been extensively applied to text modeling and
  natural language
  processing~\citep{Teh:2007,Johnson:2007,Li:2007,Blei:2003}.}  Thus,
our observations are assumed to be collections of words from a fixed
vocabulary, organized into documents.

\paragraph{Language modeling.} In the language modeling application,
each document is associated with a distance dependent CRP, and its
tables are embellished with IID draws from a base distribution over
terms or words.  (The documents share the same base distribution.)  The
generative process of words in a document is as follows.  The data are
first placed at tables via customer assignments, and then assigned to
the word associated with their tables.  Subsets of the data exhibit a
partition structure by sharing the same table.

When using a traditional CRP, this is a formulation of a simple
Dirichlet-smoothed language model.  Alternatives to this model, such
as those using the Pitman-Yor process, have also been applied in this
setting~\citep{Teh:2006a,Goldwater:2006a}.  We consider a sequential
CRP, which assumes that a word is more likely to occur near itself in
a document.  Words are still considered contagious---seeing a word
once means we're likely to see it again---but the window of contagion
is mediated by the decay function.

More formally, given a decay function $f$, sequential distances $D$,
scaling parameter $\alpha$, and base distribution $G_0$ over discrete words,
$N$ words are drawn as follows,
\begin{packed_enumerate}
\item For each word $i \in [1,N]$ draw assignment $c_i
  \sim \textrm{dist-CRP}(\alpha, f, D)$.
\item For each word $i \in [1,N]$, if $c_i \neq i$ then assign the
  word $w_i = w_{c_i}$.\\Otherwise draw the word randomly, $w_i \sim
  G_0$.
\end{packed_enumerate}
For each document, we observe a sequence of words $w_{1:N}$ from which
we can infer their seating assignments in the distance dependent CRP.
The partition structure
of observations---that is, which words are the same as other
words---indicates either that they share the same table in the seating
arrangement, or that two tables share the same term drawn from $G_0$.
We have not described the process sequentially, as one would with a
traditional CRP, in order to emphasize the two stage process of the
distance dependent CRP.  However, the sequential distances $D$
guarantee that we can draw each word successively.  This, in turn,
means that we can easily construct a predictive distribution of future
words given previous words.  (See \mysec{inference} below.)

% Note that we have described the process sequentially.  However, the
% same distribution arises by first choosing the customer assignments
% for all $N$ words, and then choosing the words based on the
% resulting seating plan.  We also study an embellishment where the
% discrete base distribution $G_0$ is endowed with a Dirichlet prior,
% thereby adding an additional level of uncertainty.

\paragraph{Mixture modeling} \label{sec:mixture-modeling}

The second model we study is akin to the CRP mixture or (equivalently)
the DP mixture, but differs in that the mixture component for a data
point depends on the mixture component for nearby data.  Again, each
table is
endowed with a draw from a base distribution $G_0$, but here that draw is a
distribution over mixture component parameters.  In the document
setting, observations are documents (as opposed to individual words),
and $G_0$ is typically a Dirichlet distribution over
distributions of words~\citep{Teh:2007}.  The data are drawn as
follows:
\begin{packed_enumerate}
\item For each document $i \in [1,N]$ draw assignment $c_i \sim
  \textrm{dist-CRP}(\alpha, f, D)$.

\item For each \DIFdelbegin \DIFdel{document $i \in [1,N]$, }\DIFdelend \DIFaddbegin \DIFadd{cluster (table) formed by the customer assignments, choose an arbitrary representative document
  $j$ from those in the cluster.  Choose the parameter for this representative document randomly, $\theta_j \sim G_0$.

}

\item \DIFadd{For each document $i \in [1,N]$,
  }\DIFaddend \begin{packed_enumerate}
  \item \DIFdelbegin \DIFdel{If $c_i \neq i$ then set the parameter for the }\DIFdelend \DIFaddbegin \DIFadd{Find the cluster in which document }\DIFaddend $i$ \DIFdelbegin \DIFdel{th
    document to $\theta_i = \theta_{c_i}$.

}%DIFDELCMD < \\
%DIFDELCMD <     %%%
\DIFdel{Otherwise choose the parameter randomly, $\theta_i \sim G_0$}\DIFdelend \DIFaddbegin \DIFadd{resides, and find the cluster's representative customer $j$.  Set $\theta_i = \theta_j$}\DIFaddend .
  \item Draw the $i$th document, $w_i \sim F(\theta_i)$.
  \end{packed_enumerate}
\end{packed_enumerate}
In \mysec{study}, we will study the sequential CRP in this setting,
choosing its structure so that contemporaneous documents are more
likely to be clustered together.  The distances $d_{ij}$ can be the
differences between indices in the ordering of the data, or lags
between external measurements of distance like date or time.  (Spatial
distances or distances based on other covariates can be used to define
more general mixtures, but we leave these settings for future work.)
Again, we have not defined the generative process sequentially but, as
long as $D$ respects the assumptions of a sequential CRP, an
equivalent sequential model is straightforward to define.

% dmb: !!! below, this might be better in the introduction or
% conclusion.  is it a little buried here?

More generally, the distance dependent CRP mixture provides an
alternative to the dependent Dirichlet process (DDP) mixture as an
infinite clustering model that models dependencies between the latent
component assignments of the data~\citep{MacEachern:1999}.  The DDP
has been extended to sequential, spatial, and other kinds of
dependence~\citep{Griffin:2006,Duan:2006,Xue:2007}.  In all these
settings, statisticians have appealed to truncations of the
stick-breaking representation for approximate posterior inference,
citing the dependency between data as precluding the more efficient
techniques that integrate out the component parameters and
proportions.  In contrast, distance dependent CRP mixtures are
amenable to Gibbs sampling algorithms that integrate out these
variables (see \mysec{inference}).

An alternative to the DDP formalism is the Bayesian density
regression (BDR) model of~\cite{Dunson:2007}.  In BDR, each data point
is associated with a random measure and is drawn from a mixture of
per-data random measures where the mixture proportions are related to
the distance between data points.  Unlike the DDP, this
model affords a Gibbs sampler where the random measures can be
integrated out.  However, it is still different in spirit from the
distance dependent CRP.  Data are drawn from distributions similar to
distributions of nearby data and thus the particular values of nearby
data impose much softer constraints than those in the distance
dependent CRP.

We emphasize that DDP mixtures (and BDR) and distance dependent CRP
mixtures are \textit{different} classes of models.  DDP mixtures are
Bayesian nonparametric models, interpretable as data drawn from a
random measure, while the distance dependent CRP mixtures generally
are not. DDP mixtures exhibit marginal invariance, while distance
dependent CRPs generally do not (see \mysec{marg}).  In their ability
to capture dependence, these two classes of models capture similar
assumptions, but the appropriate choice of model depends on the
modeling task at hand.

% \footnote{In fact, in the supplement we show that the \textit{only}
%   distance dependent CRP that is interpretable as a random measure model
%   is the traditional CRP embellished with a base measure, i.e., the
%   Dirichlet process.}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "dd-crp"
%%% End: 


==> inference.tex <==
\section{Posterior inference and prediction}
\label{sec:inference}

In both the fully-observed model (i.e., language model) and the
mixture model, our goal is to examine the posterior distribution over
partitions given a data set.  As with models based on the traditional
CRP, computing this posterior exactly is intractable.  Instead, we
approximate it using Gibbs sampling~\citep{Robert:2004}.  We construct
a Markov chain for which the stationary distribution is the posterior,
run the chain to collect samples from a close approximation to this stationary distribution,
and then use those samples to approximate the true posterior by the
empirical distribution.

\subsection{Language modeling} Recall the setting of the language
model.  Given observed words $w_{1:N}$ we are interested in the
posterior distribution of their partition, which is a by-product of
the corresponding customer assignments $c_{1:N}$.  This posterior is
then used for the predictive distribution of the next word, $p(w \g
w_{1:N})$.  The hidden variables are the customer assignments, and the
Gibbs sampler defines a chain on these variables by iteratively
sampling from the conditional distribution of each assignment given
the others and the data.

The state of the chain is a set of customer assignments $c_{1:N}$.
These assign each word $w_i$ to a customer $j$ where $j$ is either the
index of another customer or is equal to $i$.  (The case $j=i$ occurs
when the customer is not assigned to another customer.)  Assume
that $c_{-i}$ is consistent with $w_{1:N}$, in the sense that
$w_j=w_{c_j}$ for each $j\ne i$, and also assume that the distance
measurements $D$ are given.  The conditional distribution of $c_i$
given the other customer assignments $c_{-i}$, the observed data
$w_{1:N}$, and the base measure $G_0$ is,
\begin{eqnarray}
  p(c_i \g c_{-i}, w_{1:N}, G_0) &\propto&
  p(c_i \g c_{-i}, G_0) p(w_{1:N} \g c_i, c_{-i}, G_0)
  \nonumber \\
  &=& p(c_i) \ind{w_i=w_{c_i}} \textstyle \prod_{j\in R(c_{1:N})} p(w_j \mid G_0),
  \label{eq:general-obs-gibbs}
\end{eqnarray}
where $R(c_{1:N})$ is defined to contain one customer index from each
table.  For example, in \myfig{tables} this set could be $\{1, 2, 6,
10\}$.  Here we have used Bayes rule, the independence of $c_i$, and
that $p(w_{1:N} \g c_i, c_{-i})$ is the probability of independently
drawing each table's unique word from $G_0$.

The first term of \myeq{general-obs-gibbs} is the prior of
\myeq{dec-crp-prior}.  Before computing the second term, we introduce
some definitions.  First, define $R(c_{-i})$ to contain one index from
each cluster in the seating assignment $c_{-i}$ with the outgoing link
of customer $i$ removed.  (Other customers still can link to $i$, and
note that $i$ is in its own table in $R(c_{-i})$ if no other customer
links to it.)  To compute the product in \myeq{general-obs-gibbs}, we
consider the change from $R(c_{-i})$ to $R(c_{1:N})$.  That is, how
does the link $c_i$ change this set?  There are two cases: (1) The
number of tables remains the same; this occurs if customer $i$ links
to a customer that is already seated at his table. (2) Two tables are
joined; this occurs if customer $i$ links to a customer at another
table.

% To compute the second term of \myeq{general-obs-gibbs}, we now compare
% $R(c_{1:N})$ to $R(c_{-i})$ and observe that two cases are possible.  In the
% first case, $c_i$ links to a customer already in cluster $i$ under seating
% assignment $c_{-i}$ (i.e., $c_i \in S(i,c_{-i})$), in which case $R(c_{1:N}) =
% R(c_{-i})$.  In the second case, $c_i$ links to a customer outside cluster $i$
% (i.e., $c_i \notin S(i,c_{-i})$, joining these two clusters together, in which
% case $R(c_{1:N}) = R(c_{-i}) \setminus \{i\}$.  Thus, 
% \begin{equation}
% \label{eq:gibbs-tmp}
% \frac{\prod_{j\in R(c_{1:N})} p(w_j \g G_0)}{p(w_i \g G_0)\prod_{j\in R(c_{-i})} p(w_j \g G_0)} =
% \begin{cases}
% p(w_i \g G_0) & \text{if $c_i \in S(i,c_{-i})$,} \\
% 1 & \text{if $c_i \notin S(i,c_{-i})$.}
% \end{cases}
% \end{equation}

% We may consider the denominator of \myeq{gibbs-tmp} as part of the
% proportionality constant in \myeq{general-obs-gibbs}, and observing
% that $i \in S(i,c_{-i})$ we may use \myeq{dec-crp-prior} and
% \myeq{gibbs-tmp} to write

In the Gibbs sampler, there are three cases because there are two ways
of leaving the number of tables unchanged: one is by a self-link; the
other is by linking to another customer at the table.  The three cases
that result are,
\begin{equation}
\label{eq:general-obs-gibbs2}
p(c_i \g c_{-i}, w_{1:N}) \propto
\begin{cases}
  \alpha \ind{w_i=w_{c_i}} & \text{if $c_i=i$,} \\
  f(d_{ij}) \ind{w_i=w_{c_i}} & \text{if $c_i \neq i$ and $R(c_{-i})$ does not change,} \\
  f(d_{ij}) \ind{w_i=w_{c_i}}/ p(w_i \g G_0) & \text{if $c_i$ joins two tables in $R(c_{-i})$.}
\end{cases}
\end{equation}


% \begin{equation}
% \label{eq:general-obs-gibbs2}
% p(c_i \g c_{-i}, w_{1:N}) \propto
% \begin{cases}
% \alpha \ind{w_i=w_{c_i}} p(w_i \g G_0) & \text{if $c_i=i$,} \\
% f(d_{ij}) \ind{w_i=w_{c_i}} p(w_i \g G_0) & \text{if $c_i\in S(i,c_{-i})\setminus i$,} \\
% f(d_{ij}) \ind{w_i=w_{c_i}} & \text{if $c_i\notin S(i,c_{-i})$.} \\
% \end{cases}
% \end{equation}

Note that we have derived the Gibbs sampler for the general distance
based CRP, as opposed to the sequential CRP.  This sampler could be
used, for example, to cluster image codewords in a spatial setting, or
to cluster members of a social network.  Moreover, this sampler does
not hinge on discrete data; it is easily adapted to continuous data or
count data.

\paragraph{Sequential CRPs.}  In a sequential CRP, we simplify further
because the seating assignments always form an acyclic graph.  (Recall
that a customer can only choose to sit with a customer with a smaller
index and so no cycles are possible.)  In this setting, $c_i$ always
joins two tables unless it links to customer $i$.  Thus,
\begin{equation}
\label{eq:general-obs-gibbs3}
p(c_i \g c_{-i}, w_{1:N}) \propto
\begin{cases}
\alpha \ind{w_i=w_{c_i}} p(w_i \g G_0) & \text{if $c_i=i$,} \\
f(d_{ij}) \ind{w_i=w_{c_i}} & \text{if $c_i\ne i$.} \\
\end{cases}
\end{equation}
Note that we have multiplied through by $p(w_i \g G_0)$.

% dmb: i think we've handled dahl sufficiently in the earlier part of
% the paper.

% To use this Gibbs sampler to sample from the posterior resulting from
% the prior in \cite{Dahl:2008}, replace $f(d_{ij})$ with $h_{ij}$.

% for the more complex paper...

% If $c_{1:N}$ is almost surely a directed acyclic graph
% then the set of customers that may link to customer $i$, and the set
% of customers to which customer $i$ may link, have an intersection
% equal to exactly $\{i\}$.  Thus, the second case in
% \myeq{general-obs-gibbs2} may not occur, and the third case may be
% expressed as $c_i \ne i$.  Thus, in the special case of almost sure
% acyclic graphs,

\paragraph{Sampling the base distribution.}  We further consider a hierarchical
model where $G_0$ is drawn from a prior, $G_0 \sim H(\lambda)$.  Here,
the terms $p(w_i \g G_0)$ in \myeq{general-obs-gibbs2} and
\myeq{general-obs-gibbs3} must be replaced by the following integral
\begin{equation*}
  p(w_i \g c_i, c_{-i}, w_{-i}, \lambda) =
  \int p(w_i \g G_0) p(G_0 \g \{w_k : k \in R(c_{1:N})), \lambda) dG_0.
\end{equation*}
Recall, that the set $R(c_{1:N})$ contains one customer from each
partition.  In the equation, the conditional distribution of $G_0$
only depends on those data in $R(c_{1:N})$ because each table contains
exactly one draw from $G_0$.  When $H$ and $G_0$ form a conjugate
pair, this integral is a straightforward Bayesian
computation~\citep{Gelman:1995}.  For example, for a
Dirichlet-multinomial, it is the vector of normalized counts of items
drawn from $G_0$, smoothed by the scalar $\lambda$.  Note that in the
sequential CRP there are no cycles in the assignments; the set $R$ can
be obtained by taking the customers who initially sat alone.

It is also possible to place a prior on the concentration parameter
$\alpha$ and the parameters of the decay function, and then to sample them
via an augmented Gibbs sampler.  This is discussed in \myapp{hyperparams}.

\subsection{Mixture modeling}
\label{sec:mixture-inference}

We now derive the Gibbs sampler for the sequential CRP
mixture.\footnote{This algorithm generalizes to the full class of
  distance dependent CRPs as well.}  Observations are a sequence of
documents $\vec{w}_{1:N}$.  Each document contains $N$ words and is
assigned to a customer.  The Gibbs sampler iteratively draws from the
conditional distribution of each customer assignment,
\begin{equation}
  \label{eq:mixture-gibbs}
  p(c_i = j \g c_{-i}, \vec{w}_{1:N}, \alpha, D) \propto
  \left\{
    \begin{array}{ll}
      f(d_{ij})  p(\vec{w}_{1:N} \g c_{-i}, c_i = j, \lambda) &
      \textrm{if} \quad j \neq i \\
      \alpha \,  p(\vec{w}_{1:N} \g c_{-i}, c_i = i,
      \lambda) & \textrm{if} \quad j = i.
    \end{array}
  \right.
\end{equation}
Unlike a traditional CRP, the probability of the whole data set plays
a role in the case where $c_i = i$.  The posterior probability of the
assignment $c_i$ is affected by other data, e.g., future data in the
sequential setting, because some of that data might be assigned to
$c_i$.  This is not an issue in a traditional CRP mixture because the
data are exchangeable.  However, it actually is an advantage as it
allows for bigger moves in the state space.  See
\mysec{crp-comparison}.

To compute the likelihood term, again let $R(c_{1:N})$ contain one
customer index from each table, let $S_r$ be the set of customer
indices that are equal to $r$ or to any other index in $S_r$, and let
$N_{S_{r}}$ denote the word counts of documents at those indices.
Thus, if the $i$th word begins a new table then we may choose $i$ to
be in the set $R$.
If the $j$th word is assigned to $i$ and the $k$th word is assigned to
$j$, then $j$ and $k$ are both in $S_i$.  For example, $S_2$ in
\myfig{tables} is \{2,4,5,8\}.  The likelihood term is
\begin{equation}
  \textstyle p(\vec{w}_{1:N} \g c_{-i}, c_i = j, \lambda) =
  \prod_{r \in R(c_{1:N})} p(\vec{w}_{S_r} \g \lambda).
\end{equation}
When $G_0$ is conjugate to the data generating distribution, e.g.,
Dirichlet$(\lambda)$ in the case of multinomial data, each term of this
equation is a ratio of normalizing constants
(see~\citeauthor{Bernardo:1994}, \citeyear{Bernardo:1994}).
% \begin{equation}
%   \label{eq:dir-lhood}
%   p(\vec{w}_{S_r} \g c_{1:N}, \lambda) =
%   \frac{\Gamma(V\lambda)}{\Gamma(\lambda)^{V}} \cdot
%   \frac{\prod_{v=1}^V \Gamma(N_{S_r}^{(v)} + \lambda)}{\Gamma(N_{S_r}^{(\cdot)}
%     + V \lambda)},
% \end{equation}
% where $V$ is the total number of unique words in the observed data,
% $N_{S_r}^{(v)}$ is the $v$th component of the $N_{S_r}$ vector, and
% $N_{S_r}^{(\cdot)}$ denotes its sum.

Finally, note that for sequential $D$ and specific decay functions,
this provides an alternative approximate inference method for the
models of~\cite{Ahmed:2008} and~\cite{Zhu:2005}.  Moreover, since the
traditional CRP can be expressed as a sequential CRP,
\myeq{mixture-gibbs} is a new Gibbs sampler for CRP mixture models.
We compare this new sampler with the traditional collapsed Gibbs
sampler below in \mysec{crp-comparison}.

\paragraph{Prediction.} In \mysec{mixture-study}, we will assess the
log likelihood of held-out documents given a set of observed
documents, a measure of the predictive power of the model.  We
approximate this quantity from Gibbs samples.

Continue to assume that $D$ is sequential.  Let $\vec{w}$ be a held
out document, $\vec{w}_{1:N}$ be the previously observed documents,
and $c_{1:N}^{(b)}$ be the $b$th sample from a Gibbs run of $B$
samples.  The predictive likelihood is
\begin{eqnarray}
  \nonumber
  \textstyle p(\vw \g \vw_{1:N}, D, \alpha) &=&
  \nonumber
  \textstyle \sum_{c_{1:N}} p(c_{1:N} \g \vw_{1:N}, D, \alpha)
  p(\vw \g c_{1:N}, \vw_{1:N}) \\
  \nonumber
  \textstyle &\approx& \textstyle (1/B) \sum_{b=1}^{B}
  p(\vw \g c^{(b)}_{1:N}, \vw_{1:N}),
\end{eqnarray}
where each term is
\begin{equation}
  p(\vw \g c^{(b)}_{1:N}, \vw_{1:N}) =
  \sum_{c=1}^{N+1} p(c \g D, \alpha) p(\vw \g c, c^{(b)}_{1:N},
  \vw_{1:N}).
\end{equation}
The first term is the prior probability of the new customer assignment
given in \myeq{dec-crp-prior}.  (By convention, $c=N+1$ means that the
new customer sits alone.)  The conditional probability of the new
document in the second term is a ratio of probabilities: The numerator
is the marginal probability of the new document and the previous
documents assigned to the partition of $c$; the denominator is the
marginal probability of the previous documents assigned to the
partition of $c$.

When $D$ is not sequential, the predictive distribution is more
complicated---it must be estimated as a ratio of likelihoods.  This is
possible, though possibly computationally expensive, by running two
Gibbs samplers: one that includes the missing observation as a hidden
variable, and one that does not.  Other methods of estimating ratios
of likelihoods might also be available.  See, for example,
\cite{Kass:1995} and \cite{Meng:1998}.


==> proofs.tex <==
\section{Formal Characterization of Marginal Invariance}
\label{sec:formal-marg}

In this section, we formally characterize the class of distance
dependent CRPs that are marginally invariant.  This family is a very
small subset of the entire set of distance dependent CRPs, containing
only the traditional CRP and variants constructed from independent
copies of it.  This characterization is used in \mysec{marg} to
contrast the distance dependent CRP with random-measure models.

Throughout this section, we assume that the decay function satisfies
a relaxed version of the triangle inequality, which uses the notation $\bar{d}_{ij}=\min(d_{ij},d_{ji})$.
We assume:
if $\bar{d}_{ij}=0$ and $\bar{d}_{jk}=0$ then $\bar{d}_{ik}=0$; and if
$\bar{d}_{ij}<\infty$ and $\bar{d}_{jk}<\infty$ then $\bar{d}_{ik}<\infty$.

\subsection{Sequential Distances}

\newcommand{\Jfunc}{J}
\newcommand{\Jset}{\mathcal{J}}
\newcommand{\Kfunc}{k}
\newcommand{\Ksz}{K}

We first consider sequential distances.  We begin with the following proposition, which shows that a very restricted class of distance dependent CRPs may also be constructed by collections of independent CRPs. 

\begin{proposition}
  \label{p:sequential-crp}
  Fix a set of sequential distances between each of $n$ customers, a real number $a>0$, and a set $A\in\{\emptyset, \{0\}, \R\}$.  
  Then there is a (non-random) partition $B_1,\ldots,B_K$ of $\{1,\ldots,n\}$ for which two distinct customers $i$ and $j$ are in the same set $B_k$ iff $\bar{d}_{ij} \in A$.
  For each $k=1,\ldots,K$, let there be an independent CRP with concentration parameter $\alpha/a$, and let customers within $B_k$ be clustered among themselves according to this CRP.

  Then, the probability distribution on clusters induced by this construction is identical to the distance dependent CRP 
  with decay function $f(d) = a \ind{d\in A}$.  Furthermore, this probability distribution is marginally invariant.
\end{proposition}
\begin{proof}
% First partition the set of customers $\{1,\ldots,n\}$ into $K$ disjoint sets $B_1,\ldots,B_K$ so that each customer $i$ is in a single set $B_{k(i)} = \{i\} \cup \{ j\ne i : \text{ $d_{ij} \in A$ or $d_{ji}\in A$} \}$.  Such a (non-random) partition exists because of our relaxed triangle-inequality assumption, and because $A$ is either $\emptyset$, $\{0\}$, or $\infty$.  These partitions are unique, where we regard a reordering of $B_1,\ldots,B_K$ as the same partition.  
We begin by constructing a partition $B_1,\ldots,B_K$ with the stated property.
Let $\Jfunc(i) = \min\{ j : \text{$j=i$ or $\bar{d}_{ij}\in A$}\}$, and let $\Jset = \{\Jfunc(i) : i=1,\ldots,n\}$ be the set of unique values taken by $\Jfunc$.
Each customer $i$ will be placed in the set containing customer $J(i)$.
Assign to each value $j\in\Jset$ a unique integer $\Kfunc(j)$ between $1$ and $|\Jset|$.
For each $j\in\Jset$, let $B_{\Kfunc(j)} = \{ i : \Jfunc(i) = j \} = \{ i : \text{$i=j$ or $\bar{d}_{ij} \in A$} \}$.
Each customer $i$ is in exactly one set, $B_{\Kfunc(\Jfunc(i))}$, and so $B_1,\ldots,B_{|\Jset|}$ is a partition of $\{1,\ldots,n\}$.

To show that $i\ne i'$ are both in $B_k$ iff $\bar{d}_{ii'} \in A$, we consider two possibilties.  
If $A=\emptyset$, then $\Jfunc(i) = i$ and each $B_k$ contains only a single point.
If $A=\{0\}$ or $A=\R$, then it follows from the relaxed triangle inequality assumed at the beginning of Appendix~\ref{sec:formal-marg}.

With this partition $B_1,\ldots,B_K$, the probability of linkage under the
distance dependent CRP with decay function $f(d) = a \ind{d\in A}$ may be written
\begin{equation*}
p(c_i = j) \propto
\begin{cases}
\alpha & \text{if $i=j$,} \\
a & \text{if $j<i$ and $j\in B_{\Kfunc(i)}$,} \\
0 & \text{if $j>i$ or $j\notin B_{\Kfunc(i)}$.}
\end{cases}
\end{equation*}

By noting that linkages between customers from different sets $B_k$ 
occur with probability $0$, we see that this is the same probability
distribution produced by taking $K$ independent distance dependent CRPs,
where the $k$th distance dependent CRP governs linkages between
customers in $B_k$ using
\begin{equation*}
p(c_i = j) \propto
\begin{cases}
\alpha & \text{if $i=j$,} \\
a & \text{if $j<i$,} \\
0 & \text{if $j>i$,}
\end{cases}
\end{equation*}
for $i,j\in B_k$.

Finally, dividing the unnormalized probabilities by $a$, we rewrite the
linkage probabilities for the $k$th distance dependent CRP as
\begin{equation*}
p(c_i = j) \propto
\begin{cases}
\alpha/a & \text{if $i=j$,} \\
1 & \text{if $j<i$,} \\
0 & \text{if $j>i$,}
\end{cases}
\end{equation*}
for $i,j\in B_k$.  This is identical to the distribution of the traditional CRP with concentration parameter $\alpha/a$.

This shows that the distance dependent CRP with decay function
$f(d)=a\ind{d\in A}$ induces the same probability distribution on
clusters as the one produced by a collection of $K$ independent
traditional CRPs, each with concentration parameter $\alpha/a$, where
the $k$th traditional CRP governs the clusters of customers within
$B_k$.

The marginal invariance of this distribution follows from the marginal invariance of each traditional CRP, and their independence from one another.
\end{proof}


The probability distribution described in this proposition separates
customers into groups $B_1,\ldots,B_K$ based on whether inter-customer
distances fall within the set $A$, and then governs clustering within
each group independently using a traditional CRP.  Clustering across
groups does not occur.

We consider what this means for specific choices of $A$.  If $A=\{0\}$,
then each group contains those customers whose distance from one another
is $0$.  This group is well-defined because of the assumption that
$d_{ij}=0$ and $d_{jk}=0$ implies $d_{ik}=0$. If $A=\R$, then each group
contains those customers whose distance from one another is finite.
Similarly to the $A=\{0\}$ case, this group is well-defined because of
the assumption that $d_{ij}<\infty$ and $d_{jk}<\infty$ implies
$d_{ik}<\infty$.  If $A=\emptyset$, then each group contains only a
single customer.  In this case, each customer will be in his own cluster.


Since the resulting construction is marginally invariant,
Proposition~\ref{p:sequential-crp} provides a sufficient condition for
marginal invariance.  The following proposition shows that this
condition is necessary as well.

\begin{proposition}
  \label{p:sequential-marginal-invariance}
  If the distance dependent CRP for a given decay function $f$ is
  marginally invariant over all sets of sequential distances then $f$ is
  of the form $f(d) = a \ind{d\in A}$ for some $a>0$ and $A$ equal to
  either $\emptyset$, $\{0\}$, or $\R$.
\end{proposition}
\begin{proof}
Consider a setting with $3$ customers, in which customer $2$ may either be
absent, or present with his seating assignment marginalized out.  Fix a
non-decreasing decay function $f$ with $f(\infty)=0$ and suppose that the
distances are sequential, so $d_{13}=d_{23}=d_{12}=\infty$.  Suppose that the
distance dependent CRP resulting from this $f$ and any collection of sequential
distances is marginally invariant.  Then the probability that customers $1$
and $3$ share a table must be the same whether customer $2$ is absent or
present.

If customer $2$ is absent,
\begin{equation}
\label{eq:2absent}
\Prob{\text{$1$ and $3$ sit at same table} \mid \text{$2$ absent}}
= \frac{f(d_{31})}{f(d_{31}) + \alpha}.
\end{equation}

If customer $2$ is present, customers $1$ and $3$ may sit at the same
table in two different ways: $3$ sits with $1$ directly ($c_3=1$); or $3$
sits with $2$, and $2$ sits with $1$ ($c_3=2$ and $c_2=1$).  Thus,
\begin{multline}
\label{eq:2present}
\Prob{\text{$1$ and $3$ sit at same table} \mid \text{$2$ present}}\\
= \frac{f(d_{31})}{f(d_{31}) + f(d_{32}) + \alpha}
+ \left(\frac{f(d_{32})}{f(d_{31}) + f(d_{32}) + \alpha}\right)
  \left(\frac{f(d_{21})}{f(d_{21}) + \alpha}\right).
\end{multline}

For the distance dependent CRP to be marginally invariant,
\myeq{2absent} and \myeq{2present} must be identical.  Writing
\myeq{2absent} on the left side and \myeq{2present} on the right, we
have
\begin{equation}
\frac{f(d_{31})}{f(d_{31}) + \alpha}
= \frac{f(d_{31})}{f(d_{31}) + f(d_{32}) + \alpha}
+ \left(\frac{f(d_{32})}{f(d_{31}) + f(d_{32}) + \alpha}\right)
  \left(\frac{f(d_{21})}{f(d_{21}) + \alpha}\right).
\label{eq:equality}
\end{equation}

We now consider two different possibilities for the distances $d_{32}$ and $d_{21}$, always keeping $d_{31}=d_{21}+d_{32}$.

%In the first case, suppose $d_{32} = d_{21} = 0$.  By
%multiplying \myeq{2present} through by 
%$\left[2f(0) + \alpha\right]\left[f(0)+\alpha\right]$ 
%and rearranging terms, we obtain
%\begin{equation*}
%  0 = f(0)\left[ \alpha - f(0) \right].
%\end{equation*}
%Thus, we either have $f(0)=0$ or $f(0)=\alpha$.  If $f(0)=0$, then $f$ nonincreasing implies that $f$ is identically $0$, which is of the form claimed by the proposition, with $A=\emptyset$.  We may then continue under the assumption that $f(0)=\alpha$.  

First, suppose $d_{21} = 0$ and $d_{32} = d_{31} = d$ for some $d\ge 0$.
By multiplying \myeq{equality} through by 
$\left(2f(d) + \alpha\right)\left(f(0)+\alpha\right)\left(f(d)+\alpha\right)$ 
and rearranging terms, we obtain
\begin{equation*}
  0 = \alpha f(d)\left( f(0) - f(d) \right).
\end{equation*}
Thus, either $f(d)=0$ or $f(d)=f(0)$.  Since this is true for each
$d\ge0$ and $f$ is nonincreasing, $f=a\ind{d\in A}$ with $a\ge0$ and either $A=\emptyset$, $A=\R$, $A=[0,b]$, or $A=[0,b)$ with $b\in[0,\infty)$.  Because $A=\emptyset$ is among the choices, we may assume $a>0$ without loss of generality.  We now show that if $A=[0,b]$ or $A=[0,b)$, then we must have $b=0$ and $A$ is of the form claimed by the proposition.

Suppose for contradiction that $A=[0,b]$ or $A=[0,b)$ with $b>0$.  
Consider distances given by $d_{32}=d_{21}=d=b-\epsilon$ with $\epsilon\in(0,b/2)$.  
By multiplying
\myeq{2present} through by 
\begin{equation*}
  \left(f(2d) + f(d) + \alpha\right)\left(f(d)+\alpha\right)\left(f(2d)+\alpha\right)
\end{equation*}
and rearranging terms, we obtain
\begin{equation*}
  0 = \alpha f(d)\left( f(d) - f(2d) \right).
\end{equation*}
Since  $f(d)=a>0$, we must have $f(2d)=f(d)>0$.
But, $2d = 2(b - \epsilon) > b$ implies together with $f(2d) = a \ind{2d\in A}$
that $f(2d)=0$, which is a contradiction.
\end{proof}

These two propositions are combined in the following corollary, which
states that the class of decay functions considered in
Propositions~\ref{p:sequential-crp}
and~\ref{p:sequential-marginal-invariance} is both necessary and
sufficient for marginal invariance.

\begin{corollary}
  \label{c:sequential-not-marg}
  Fix a particular decay function $f$.
  The distance dependent CRP resulting from this decay function is marginally invariant over all sequential distances if and only if $f$ is of the form $f(d) = a\ind{d\in A}$ for some $a>0$ and some $A\in\{\emptyset, \{0\}, \R\}$.
\end{corollary}
\begin{proof}
  Sufficiency for marginal invariance is shown by Proposition~\ref{p:sequential-crp}.  Necessity is shown by Proposition~\ref{p:sequential-marginal-invariance}.
\end{proof}


Although Corollary~\ref{c:sequential-not-marg} allows any choice of $a>0$ in the decay function $f(d)=a\ind{d\in A}$, the distribution of the distance dependent CRP with a particular $f$ and $\alpha$ remains unchanged if both $f$ and $\alpha$ multiplied by a constant factor (see \myeq{dec-crp-prior}).  Thus, the distance dependent CRP defined by $f(d)=a\ind{d\in A}$ and concentration parameter $\alpha$ is identical to the one defined by $f(d)=\ind{d\in A}$ and concentration parameter $\alpha/a$.  In this sense, we can restrict the choice of $a$ in Corollary~\ref{c:sequential-not-marg} (and also Propositions~\ref{p:sequential-crp} and~\ref{p:sequential-marginal-invariance})
to $a=1$ without loss of generality.






% A word of explanation about the distribution induced:
% The distribution induced is the same as created by a collection of
% independent CRPs.  Each independent CRP is placed on a collection of
% customers whose distances from each other fall within $A$.

\subsection{General Distances}

We now consider all sets of distances, including non-sequential
distances.  The class of distance dependent CRPs that are marginally
invariant over this larger class of distances is even more restricted
than in the sequential case.  We have the following proposition
providing a necessary condition for marginal invariance.

\begin{proposition}
  \label{p:general-marginal-invariance}
  If the distance dependent CRP for a given decay function $f$ is
  marginally invariant over all sets of distances, both sequential and
  non-sequential, then $f$ is identically $0$.
\end{proposition}
\begin{proof}
  From Proposition~\ref{p:sequential-marginal-invariance}, we have that any decay function that is marginally invariant under all sequential distances must be of the form $f(d) = a \ind{d\in A}$, where $a>0$ and $A\in\{\emptyset,\{0\},\R\}$.  We now show that if the decay function is marginally invariant under {\it all} sets of distances (not just those that are sequential), then $f(0)=0$.  The only decay function of the form $f(d) = a \ind{d\in A}$ that satisfies $f(0)=0$ is the one that is identically $0$, and so this will show our result.

  To show $f(0) = 0$, suppose that we have $n+1$ customers, all of whom are a distance $0$ away from one another, so $d_{ij}=0$ for $i,j=1,\ldots,n+1$.  Under our assumption of marginal invariance, the probability that the first $n$ customers sit at separate tables should be invariant to the absence or presence of customer $n+1$. 

  When customer $n+1$ is absent, the only way in which the first $n$
  customers may sit at separate tables is for each to link to himself.
  Let $p_n = \alpha / (\alpha + (n-1)f(0))$ denote the probability of a
  given customer linking to himself when customer $n+1$ is absent.
  Then 
  \begin{equation}
    \label{eq:general-distance-proof-absent}
    \Prob{\text{$1,\ldots,n$ sit separately} \mid \text{$n+1$ absent}}
    = (p_n)^n.
  \end{equation}

  We now consider the case when customer $n+1$ is present.  Let $p_{n+1}
  = \alpha / (\alpha+nf(0))$ be the probability of a given customer
  linking to himself, and let $q_{n+1} = f(0) / (\alpha+nf(0))$ be the
  probability of a given customer linking to some other given customer.
  The first $n$ customers may each sit at separate tables in two
  different ways.  First, each may link to himself, which occurs
  with probability $(p_{n+1})^n$.  Second, all but one of these first
  $n$ customers may link to himself, with the remaining customer
  linking to customer $n+1$, and customer $n+1$ linking either to
  himself or to the customer that linked to him.  This
  occurs with probability $n (p_{n+1})^{n-1} q_{n+1} (p_{n+1} +
  q_{n+1})$.
  Thus, the total probability that the first $n$ customers sit at separate tables is 
  \begin{equation}
    \label{eq:general-distance-proof-present}
    \begin{split}
    \Prob{\text{$1,\ldots,n$ sit separately} \mid \text{$n+1$ present}}
    = (p_{n+1})^n + n (p_{n+1})^{n-1} q_{n+1} (p_{n+1} + q_{n+1}).
    \end{split}
  \end{equation}

  Under our assumption of marginal invariance,
  \myeq{general-distance-proof-absent} must be equal to
  \myeq{general-distance-proof-present}, and so 
  \begin{equation}
    \label{eq:general-distance-polynomial}
    0 = (p_{n+1})^n + n (p_{n+1})^{n-1} q_{n+1} (p_{n+1} + q_{n+1}) - (p_n)^n.
  \end{equation}

  Consider $n=2$.  By substituting the definitions of $p_2$, $p_3$, and $q_3$, and then rearranging terms, we may rewrite \myeq{general-distance-polynomial} as
  \begin{equation*}
    0 = \frac{\alpha f(0)^2  (2f(0)^2 - \alpha^2)}{(\alpha+f(0))^2 (\alpha+2f(0))^3},
  \end{equation*}
  which is satisfied only when $f(0) \in \{0, \alpha/\sqrt{2}\}$.  Consider the second of these roots, $\alpha/\sqrt{2}$.  When $n=3$, this value of $f(0)$ violates \myeq{general-distance-polynomial}.  Thus, the first root is the only possibility and we must have $f(0) = 0$.

\end{proof}

The decay function $f=0$ described in
Proposition~\ref{p:general-marginal-invariance} is a special case of
the decay function from
Proposition~\ref{p:sequential-marginal-invariance}, obtained by taking
$A=\emptyset$.  As described above, the resulting probability
distribution is one in which each customer links to himself, and is
thus clustered by himself.  This distribution is marginally invariant.
From this observation quickly follows the following corollary.

\begin{corollary}
  \label{c:general-not-marg}
  The decay function $f=0$ is the only one for which the resulting
  distance dependent CRP is marginally invariant over all distances,
  both sequential and non-sequential.  
\end{corollary}
\begin{proof}
Necessity of $f=0$ for marginal invariance follows from Proposition~\ref{p:general-marginal-invariance}.  Sufficiency follows from the fact that the probability distribution on partitions induced by $f=0$ is the one under which each customer is clustered alone almost surely, which is marginally invariant.
\end{proof}









% dmb: note that this can be used on $a$ as well.

% Or, one may choose a discrete approximation to the desired prior
% $p(\alpha)$ that is concentrated on a finite set, evaluate and
% normalize \eqref{eq:posterior_alpha} or
% \eqref{eq:posterior_alpha_window} on this set, and sample exactly
% from the approximate posterior induced by this approximate prior.

\section{Gibbs sampling for the hyperparameters}
\label{app:hyperparams}

To enhance our models, we place a prior on the concentration parameter
$\alpha$ and augment our Gibbs sampler accordingly, just as is done in
the traditional CRP mixture~\citep{Escobar:1995}.  To sample from the
posterior of $\alpha$ given the customer assignments $c_{1:N}$ and
data, we begin by noting that $\alpha$ is conditionally independent of
the observed data given the customer assignments.  Thus, the quantity
needed for sampling is
\begin{equation*}
  p(\alpha \g c_{1:N}) \propto p(c_{1:N}\g \alpha) p(\alpha),
\end{equation*}
where $p(\alpha)$ is a prior on the concentration parameter.

From the independence of the $c_i$ under the generative process, we observe
that $p(c_{1:N}\g \alpha) = \prod_{i=1}^N p(c_{i} \g D, \alpha)$.  Normalizing
provides
\begin{align*}
  p(c_{1:N}\g \alpha) &= \prod_{i=1}^N \frac{\ind{c_i=i}\alpha +
    \ind{c_i\ne
      i}f(d_{ic_i})}{\alpha + \sum_{j \neq i} f(d_{ij})}\\
  &\propto \alpha^{|R|} \left[\prod_{i=1}^N \left(\alpha +
      \sum_{j \neq i} f(d_{ij})\right)\right]^{-1},
\end{align*}
and so
\begin{equation}
  \label{eq:posterior_alpha}
  p(\alpha \g c_{1:N})
  \propto \alpha^{|R|} \left[\prod_{i=1}^N \left(\alpha +
      \sum_{j \neq i} f(d_{ij})\right)\right]^{-1} p(\alpha).
\end{equation}

% pif: This paragraph (to the blank line below) was commented out
% previously.  Was this just for space requirements in the NIPS paper,
% or should it still be commented out?  The equation eq:window_term is
% used in the Sampling decay function hyperparameters section of the
% appendix.

% dmb: i like this paragraph; lets leave it in.

When $f$ is the window decay function, $f(d) = \ind{d<a}$, and
$d_{ij}=i-j$, \myeq{posterior_alpha} reduces further.  In this
case, $\sum_{j=1}^{i-1} f(d_{ij}) = (i-1)\wedge(a-1)$, where $\wedge$
is the minimum operator, and
 \begin{equation}
   \label{eq:window_term}
   \prod_{i=1}^N \left(\alpha + \sum_{j=1}^{i-1} f(d_{ij})\right) =
   (\alpha+a-1)^{[N-a]^+} \Gamma(\alpha+a\wedge N)/\Gamma(\alpha),
 \end{equation}
 where $[N-a]^+=\max(0,N-a)$ is the positive part of $N-a$.  Then,
 \begin{equation}
   \label{eq:posterior_alpha_window}
   p(\alpha \g c_{1:N})
   \propto \frac{\Gamma(\alpha)}{\Gamma(\alpha+a\wedge
     N)}\frac{\alpha^{|R|}}{(\alpha+a-1)^{[N-a]^+}}p(\alpha).
 \end{equation}

 If we use the decay function that results in the traditional CRP,
 then we recover an expression from \cite{Antoniak:1974}, $p(\alpha \g
 c_{1:N}) \propto
 \frac{\Gamma(\alpha)}{\Gamma(\alpha+N)}\alpha^{|R|}p(\alpha)$.  This
 expression is used in \cite{Escobar:1995} to sample exactly from the
 posterior of $\alpha$ when the prior is gamma distributed.

In general, if the prior on $\alpha$ is continuous then it is
difficult to sample exactly from the posterior of
\myeq{posterior_alpha}.  There are a number of ways to address this.
We may, for example, use the Griddy-Gibbs method~\citep{Ritter:1992}.
This method entails evaluating \myeq{posterior_alpha} on a finite set
of points, approximating the inverse cdf of $p(\alpha \g c_{1:N})$
using these points, and transforming a uniform random variable with
this approximation to the inverse cdf.

We may also sample over any hyperparameters in the decay function
used, e.g., the window size in the window decay function, or the rate
parameter in the exponential decay function.  For the rest of this
section, we use $a$ to generically denote a hyperparameter in the
decay function, and we make this dependence explicit by writing
$f(d,a)$ in this section.

To describe sampling over these hyperparameters in the decay function,
we first write
 \begin{align*}
   p(c_{1:N}\mid \alpha,a)
   &= \prod_{i=1}^N \frac{\ind{c_i=i}\alpha + \ind{c_i\ne i}f(d_{ic_i},a)}{\alpha + \sum_{j=1}^{i-1} f(d_{ij},a)}\\
   &= \alpha^{|R|} \left[\prod_{i\notin R} f(d_{ij},a)\right]
   \left[\prod_{i=1}^N \left(\alpha + \sum_{j=1}^{i-1}
       f(d_{ij},a)\right)\right]^{-1}.
 \end{align*}

 Since $a$ is conditionally independent of the observed data given
 $c_{1:N}$ and $\alpha$, to sample over $a$ in our Gibbs sampler it is
 enough to know the density
 \begin{equation}
 \label{eq:posterior_a}
 p(a\mid c_{1:N},\alpha)
 \propto
 \left[\prod_{i\notin R} f(d_{ij},a)\right]
 \left[\prod_{i=1}^N \left(\alpha + \sum_{j=1}^{i-1} f(d_{ij},a)\right)\right]^{-1}
 p(a\mid \alpha).
 \end{equation}
 In many cases our prior on $a$, $p(a\mid\alpha)$, will be independent
 of $\alpha$.

 In the case of the window decay function with $d_{ij}=i-j$, we can
 simplify this further as we did above with \myeq{window_term}.  
 Noting that $\prod_{i\notin R} f(d_{ij},a)$ will be
 $1$ for those $a>\max_i i-c_i$, and $0$ for other $a$, we have
 \begin{equation}
   p(a\mid c_{1:N},\alpha)
   \propto
   \frac{\Gamma(\alpha)}{\Gamma(\alpha+a\wedge N)}\frac{p(a\mid
     \alpha)\ind{a>\max_i i-c_i}}{(\alpha+a-1)^{[N-a]^+}}.
 \end{equation}

 If the prior distribution on $a$ is discrete and concentrated on a
 finite set, as it might be with the window decay function, one can
 simply evaluate and normalize \myeq{posterior_a} on this set.  If
 the prior is continuous, as it would likely be with the exponential
 decay function, then it is difficult to sample exactly from
 \myeq{posterior_a}, but one can again use the Griddy-Gibbs
 approach of \cite{Ritter:1992} to sample approximately.
 % Or approximate $p(a\mid\alpha)$ with a discrete distribution and
 % sample from the induced approximate posterior.

